Mitigating Architectural Mismatch During the Evolutionary Synthesis of Deep Neural Networks

Evolutionary deep intelligence has recently shown great promise for producing small, powerful deep neural network models via the organic synthesis of increasingly efficient architectures over successive generations. Existing evolutionary synthesis processes, however, have allowed the mating of parent networks independent of architectural alignment, resulting in a mismatch of network structures. We present a preliminary study into the effects of architectural alignment during evolutionary synthesis using a gene tagging system. Surprisingly, the network architectures synthesized using the gene tagging approach resulted in slower decreases in performance accuracy and storage size; however, the resultant networks were comparable in size and performance accuracy to the non-gene tagging networks. Furthermore, we speculate that there is a noticeable decrease in network variability for networks synthesized with gene tagging, indicating that enforcing a like-with-like mating policy potentially restricts the exploration of the search space of possible network architectures.

==> Background.tex <==
Previous studies~\cite{Angeline1994, Stanley2002, Stanley2005, Gauci2007, Tirumala2016} have been conducted that leverage the idea of using evolutionary techniques to generate and train neural networks. In 1994, Angeline~\textit{et al.}~\cite{Angeline1994} introduced an evolutionary program GNARL (GeNeralized Acquisition of Recurrent Links) that nonmonotonically constructs recurrent networks. The GNARL algorithm simultaneously acquires the structure and weights of networks, minimizing network architectural restrictions and avoiding structural hill climbing. 

Stanley~\textit{et al.}~\cite{Stanley2002} proposed NeuroEvolution of Augmenting Topologies (NEAT) to investigate the advantage of evolving neural network topologies along with weights. NEAT resulted in faster learning and increased network efficiency by employing a principled crossover method of varying topologies, protecting structural innovation, and incrementally growing networks from minimal structure.

Stanley~\textit{et al.}~\cite{Stanley2005} extended the previous work to real-time NeuroEvolution of Augmenting Topologies (rtNEAT) for evolving increasingly complex neural networks real-time during a Neuroevolving Robotics Operatives (NERO) game in which a player trains a team of virtual robots for combat against other players' teams. The rtNEAT method allows agents to change and evolve increasingly sophisticated behaviours in real time by continually replacing poorly performing agents with new agents while preserving speciation dynamics.

Gauci and Stanley~\cite{Gauci2007} further extended this research to HyperNEAT, a Hypercube-based NeuroEvolution of Augmenting Topologies method. HyperNEAT evolves a generative encoding called connective Compositional Pattern Producing Networks (connective CPPNs) to discover geometric regularities in the application domain. HyperNEAT uses NEAT to evolve CPPNs that represent spatial patterns, with the aim of encoding connectivity patterns to evolve large-scale neural networks.

Most recently, Tirumala~\textit{et al.}~\cite{Tirumala2016} proposed a prospect for evolving network architectures that can reduce training time and provide a warm start to the deep learning process by using optimized deep neural networks as a starting point rather than a randomly initialized architecture. Using two populations of networks where one population evolves using competitive co-evolution and the other population evolves using cooperative co-evolution, the approach uses two different types of co-evolutionary processes by implementing a migration process between the two network populations after a few generations, and encourages combinations with networks from different populations to create more diversity. 
